A formal approach for correct-by-construction system substitution

The substitution of a system with another one may occur in several situations like system adaptation, system failure management, system resilience, system reconfiguration, etc. It consists in replacing a running system by another one when given conditions hold. This contribution summarizes our proposal to define a formal setting for proving the correctness of system substitution. It relies on refinement and on the Event-B method.

==> Makefile <==
LATEX = latex # -interaction=batchmode
BIBTEX = bibtex -terse

COLOR_RED    = \033[0;31m
COLOR_GREEN  = \033[0;32m
COLOR_YELLOW = \033[0;33m
COLOR_BLUE   = \033[0;34m
COLOR_CYAN   = \033[0;36m
COLOR_END    = \033[0m

all: paper.pdf

auto:
	latexmk -pdf -pvc

paper.dvi: paper.tex ../../bibliographie/database.bib
	@printf   "${COLOR_YELLOW}-= LaTeX =-${COLOR_END}\n"
	${LATEX}   paper.tex
	@printf "\n${COLOR_YELLOW}-= BibTeX =-${COLOR_END}\n"
	${BIBTEX}  paper.aux
	@printf "\n${COLOR_YELLOW}-= LaTeX =-${COLOR_END}\n"
	${LATEX}   paper.tex
	@printf "\n${COLOR_YELLOW}-= LaTeX =-${COLOR_END}\n"
	${LATEX}   paper.tex

paper.pdf: paper.dvi
	@printf "\n${COLOR_YELLOW}-= DVI->PDF =-${COLOR_END}\n"
	dvipdfmx -p letter paper.dvi

clean:
	rm -f *.dvi
	rm -f *.aux *.log *.nav *.out *.snm *.toc *.dvi *.bbl *.blg *.fls
	rm -f *.fdb_latexmk *.synctex* *.ilg *.nlo *.nls

